SIMD-PAC-DB: Pretty Performant PAC Privacy

This work presents a highly optimized implementation of PAC-DB, a recent and promising database privacy model. We prove that our SIMD-PAC-DB can compute the same privatized answer with just a single query, instead of the 128 stochastic executions against different 50% database sub-samples needed by the original PAC-DB. Our key insight is that every bit of a hashed primary key can be seen to represent membership of such a sub-sample. We present new algorithms for approximate computation of stochastic aggregates based on these hashes, which, thanks to their SIMD-friendliness, run up to 40x faster than scalar equivalents. We release an open-source DuckDB community extension which includes a rewriter that PAC-privatizes arbitrary SQL queries. Our experiments on TPC-H, Clickbench, and SQLStorm evaluate thousands of queries in terms of performance and utility, significantly advancing the ease of use and functionality of privacy-aware data systems in practice.

==> sections/deprecated3_non_resampling.tex <==

\color{red}

\section{PAC-Private Relational Algebra}
In this section, we formalize the query semantics of our PAC-privatized engine, SIMD-PAC-DB. To establish a rigorous foundation, we first present a relational-algebra formalization of a baseline execution model under the PAC-DB approach~\cite{sridhar2026pacdb} that materializes the $m$ possible worlds, and state formal privacy guarantees. In particular, because our framework maintains a persistent secret across all cells, it yields stronger concrete privacy bounds for composed queries than the independent resampling approach of PAC-DB under query-level MIAs. We then introduce the semantics of SIMD-PAC-DB, demonstrating how to vectorize this process into a single, highly efficient query. Crucially, we prove that SIMD-PAC-DB is computationally equivalent to the materialized baseline, computing the exact same variances and noise without the overhead of realizing $m$ physical worlds. To provide a formal and concise characterization, our analysis focuses on a broad class of queries supported by our system; however, it may not capture the full spectrum of queries it is capable of handling.

% a bit redundant considering much of it are defined in sec 2 already
\vspace*{2mm}
\noindent
\textbf{Notations.} Let $U$ denote the designated privacy unit (PU) table with primary key attribute~$\mathsf{pk}_U$.
A base relation~$T$ may be linked to~$U$ through a foreign key chain $T \xrightarrow{fk_1} T_1 \xrightarrow{fk_2} T_2 \cdots \xrightarrow{fk_k} U$; each tuple $t \in T$ is then associated with exactly one PU identifier, which we denote $\mathsf{pu}(t)$, obtained by following the foreign key path.
We define a mapping $\mathsf{PACLink}$ that associates each base relation 
with its corresponding foreign-key chain leading to the PU table~$U$. 
If a base relation $T$ is not linked to $U$ through any such chain, 
we define $\mathsf{PACLink}(T) = \perp$. 
We write $m$ for the number of subsets and $B$ for the per-cell mutual information (MI) budget. We adopt a hash function $H : \mathrm{dom} \to \{0,1\}^m$
and write $H(x)[j]$ for the $j$-th bit of $H(x)$, where $1 \le j \le m$. Further, given $m$ values $y_1, \ldots, y_m$, we write
$\mathsf{Var}_{\mathrm{emp}}(y_1, \ldots, y_m)
= \frac{1}{m-1}\sum_{i=1}^{m}(y_i - \bar{y})^2$
for their empirical variance, and $k \xleftarrow{\$} [1,m]$ for uniform random selection from $\{1,2,\ldots,m\}$.

\subsection{Semantics for PAC-Private Databases}
To formally describe the baseline materialized-worlds framework, we introduce three auxiliary functions and expressions.

\vspace*{2mm}
\noindent
\textbf{LinkPU$(I)$:}
Given a base relation $I$, this function augments $I$ with the privacy-unit attribute $\mathsf{pu}$. Specifically, it follows the foreign-key chain specified in $\mathsf{PACLink}[I]$, joining $I$ to the privacy-unit table $U$ through a sequence of equi-join operations along $fk = pk$ relationships. After performing these joins, the function applies the projection $\pi_{\{\mathsf{pu}\} \cup \mathsf{Attr}(I)}$ to the resulting relation. In the updated relation $I'$, the attribute $\mathsf{pu}$ records the ownership associated with each tuple in $I$. If $\mathsf{PACLink}[I] = \perp$, the function simply returns $I$ unchanged.

\vspace*{2mm}
\noindent
\textbf{SamplePU$(U)$:}
This function outputs $m$ sampled instances of the privacy-unit table $U$, denoted by $\{S_i\}_{i=1}^m$, alongside a single, uniformly sampled secret subset index $j^* \stackrel{\$}{\leftarrow} \{1, \ldots, m\}$. It also initializes a global probability vector $P \in \mathbb{R}^m$, representing the prior distribution over the subsets, to a uniform distribution $P = (1/m, \ldots, 1/m)$. The sampled index $j^*$ acts as the persistent secret, and $P$ acts as the persistent state across the entire query execution.

\vspace*{2mm}
\noindent
\textbf{Noise function pdbnoise}$(\mathsf{col}, j^*, B) \rightarrow \mathbb{R}$:
This stateful function is used within the aggregation operator $\gamma$. It takes as input a column $\mathsf{col}$ consisting of $m$ values $y_1, \ldots, y_m$, the globally sampled secret index $j^*$, and a per-cell MI budget $B$. It executes the following steps:
\begin{enumerate}[leftmargin=*]
    \item Computes the variance of the outputs weighted by the current global distribution $P$: $s^2 \leftarrow \mathsf{Var}_{P}(y_1, \ldots, y_m)$.
    \item Sets the calibrated noise variance $\Delta \leftarrow s^2/(2B)$.
    \item Outputs $\widetilde{y} \leftarrow y_{j^*} + \mathcal{N}(0, \Delta)$.
    \item Performs a Bayesian update on the global vector $P$ given the observation $\widetilde{y}$:
    $P \leftarrow (P \odot W)/\mathsf{sum}(P\odot W)$,
    where $\odot$ denotes element-wise multiplication and $W \in \mathbb{R}^m$ is the likelihood vector with elements $W_i = \exp(-(\widetilde{y} - y_i)^2/(2\Delta))$.
\end{enumerate}

Let $\mathbb{I} = \{I_1, \ldots, I_n\}$ denote the set of base relations. For each sensitive relation $I_j$, we assume that it has been augmented with the privacy-unit attribute $\mathsf{pu}$ via the transformation
$I_j := \mathsf{LinkPU}(I_j)$ for all $ 1 \leq j \leq n$. Non-sensitive relations remain unchanged.
Let $Q^{\mathsf{pdb}}(\mathbb{I})$ denote the class of queries of the form
\[
Q^{\mathsf{pdb}}(\mathbb{I})
:=
\pi_{G,\; \mathsf{f}_1 \rightarrow \alpha_1, \ldots, \mathsf{f}_c \rightarrow \alpha_c}
\;
\sigma_{\mathsf{p}}
\big(
\gamma_{G;\; \mathsf{Aggs}}(T_s)
\big),
\]
where $T_s$ is the output of an arbitrary subquery over $\mathbb{I}$, $G$ is a set of grouping attributes, $\mathsf{Aggs}$ is a list of aggregation functions,
$\mathsf{p}$ is a predicate defined over the aggregation results, and each $\mathsf{f}_i$ is an expression over aggregation outputs for $1 \leq i \leq c$. Given such a query, the baseline engine produces the PAC-private query result $\widetilde{Q}^{\mathsf{pdb}}(\mathbb{I})$
through the following compilation procedure.

\noindent \textbf{(1) Generate $m$ sampled database instances and initialize state.} Let $\left(\{S_i\}_{i=1}^{m}, j^*, P\right) := \mathsf{SamplePU}(U)$. For each relation $I_j$ and each sample index $i$, we define
\[
I_j^{(i)} :=
\begin{cases}
I_j \Join_{\mathsf{pu}} S_i, 
& \text{if } \mathsf{pu} \in \mathsf{Attr}(I_j), \\[0.5em]
I_j, 
& \text{otherwise},
\end{cases}
\quad
1 \leq j \leq n,\; 1 \leq i \leq m.
\]
The $i$-th sampled database instance is then defined as $\mathbb{I}^{(i)} := \{\, I_j^{(i)} \mid 1 \leq j \leq n \,\}$.

\noindent
\textbf{(2) Execute $m$ queries, retain stable group cells, and add noise.}
First, evaluate the query on each sampled instance and take the multiset union:
\[
T_1 
:= 
\uplus_{i=1}^{m}
Q^{\mathsf{pdb}}(\mathbb{I}^{(i)}).
\]
Next, retain only those group-by cells that appear in all $m$ runs:
\[
T_2 
:=
T_1 
\Join_{G}
\pi_{G}(
\sigma_{cnt = m}
(\gamma_{G;\; \mathsf{count}(*) \rightarrow cnt}(T_1))).
\]
Finally, apply the noise mechanism to each aggregated attribute using the persistent secret $j^*$ and a designated budget $B$:
\[
\widetilde{Q}^{\mathsf{pdb}}(\mathbb{I})
:=
\gamma_{G;\;
\mathsf{pdbnoise}(\alpha_1, j^*, B), \ldots,
\mathsf{pdbnoise}(\alpha_c, j^*, B)
}(T_2).
\]

\vspace*{2mm}
\noindent
\textbf{Privacy Guarantee.} By adaptively calibrating the injected noise to the conditional variance across the $m$ sampled instances, this compilation procedure rigorously bounds the adversarial advantage.

\begin{theorem}[Posterior Advantage Bound~\cite{zhu2026pacadversarial}]\label{thm:post_adv}
For any arbitrary inference attack and an arbitrary informed adversary $A$, let $1-\delta_0$ denote the prior success rate and $1-\delta_A$ denote the posterior success rate after observing $\widetilde{Q}^{\mathsf{pdb}}(\mathbb{I})$. The adversary's posterior advantage is strictly bounded by:
$D_{\mathrm{KL}}(\bm{1}_{1-\delta_0} \,\|\, \bm{1}_{1-\delta_A}) \leq I(j^*;\widetilde{Q}^{\mathsf{pdb}}(\mathbb{I})) \leq cB$.
\end{theorem}

While Theorem~\ref{thm:post_adv} holds generically for any subset sampling strategy, instantiating $\mathsf{SamplePU}$ with a balanced subset construction where $\forall x\in U$, $|\{i:x\in S_i\}|=m/2$ ensures a clean, deterministic baseline for concrete attacks. Specifically, under balanced sampling, the prior success rate ($1-\delta_0$) for MIA on any target record is exactly $50\%$. This allows the total MI bound $cB$ to translate into the strict, concrete limits on MIA success established previously.

\vspace*{2mm}
\noindent
\textbf{Comparisons to PAC-DB.}
While the execution model presented above builds upon the physical materialization strategy of the original PAC-DB framework~\cite{sridhar2026pacdb}, it introduces critical modifications to support sound multi-cell composition via a recent adaptive composition theorem~\cite{zhu2026pacadversarial}. In its original formulation, PAC-DB does not maintain a persistent global secret $j^*$ or a stateful posterior distribution $P$. Instead, its $\mathsf{pdbnoise}$ function independently resamples a new subset index $j_k \stackrel{\$}{\leftarrow} \{1, \ldots, m\}$ for every scalar cell evaluated by the aggregation operator. Under this original model, the total MI over $c$ cells is still bounded by $cB$, yielding an identical posterior advantage bound: $D_{\mathrm{KL}}(\bm{1}_{1-\delta_A} \,\|\, \bm{1}_{1-\delta_0}) \leq I(j_1,\ldots,j_c;\widetilde{Q}^{\mathsf{pdb}}(\mathbb{I})) \leq cB$. 

While this provides equivalent protection against \emph{cell-level MIA}, where the prior remains exactly $50\%$ for any single cell in both models, the practical privacy guarantee is significantly weaker under \emph{query-level MIA}, where the adversary attempts to infer whether a target privacy unit was used to compute \emph{any} of the $c$ cells in the query result. Because original PAC-DB relies on $c$ independently sampled subsets rather than a single persistent one, the probability that a target record appears in at least one evaluated subset grows, causing the adversary's baseline prior success rate ($1-\delta_0$) to degrade rapidly toward $100\%$ as the number of cells $c$ increases. By enforcing a persistent secret $j^*$, our formulation maintains a strict $50\%$ prior for the entire query, translating the exact same MI budget into strictly stronger, concrete privacy guarantees.


==> sections/deprecated3pacra.tex <==
\section{PAC Relational Algebra}
\label{sec:algebra}
\color{red}
Dandan: ----------------------------------------------------------------------

\begin{figure*}[t]\scriptsize
\hrulefill
\begin{multicols}{2}
\begin{algorithmic}[1]
\color{red}
\Statex \textbf{PAC-noise operator}
\[
\mathcal{N}^{\mathsf{pac}(\beta)}(T_1,\ldots,T_m)
\]

\Statex \textbf{Input:}
$m$ input relations sharing the same schema.

\Statex \textbf{Output:}
A relation $R$.
\vspace{0.25em}

\State $R \leftarrow \emptyset$
\State $(G,\mathsf{attr}_1,\ldots,\mathsf{attr}_c)
\leftarrow \mathsf{GAttr}(T_1)$

\If{$G = \emptyset$}
    \State $GV \leftarrow \{\perp\}$
\Else
    \State $GV \leftarrow
    \pi_G(T_1) \Join \cdots \Join \pi_G(T_m)$
\EndIf

\For{each $g \in GV$}
    \For{$j = 1$ to $c$}
        \For{$i = 1$ to $m$}
            \If{$G = \emptyset$}
                \State $y_{i,j} \leftarrow
                \pi_{\mathsf{attr}_j}(T_i)$
            \Else
                \State $y_{i,j} \leftarrow
                \pi_{\mathsf{attr}_j}
                (\sigma_{G=g}(T_i))$
            \EndIf
        \EndFor
            \State $s^2_j \leftarrow
            \mathsf{Var}_{\mathrm{emp}}
            (y_{1,j},\ldots,y_{m,j})$
            \State $\Delta_j \leftarrow
            \dfrac{s^2_j}{2\beta}$

        \State $k \stackrel{\$}{\leftarrow} [1,m]$
            \State $\widetilde{y}_j \leftarrow
            y_{k,j} + \mathcal{N}(0,\Delta_j)$
    \EndFor

    \If{$G = \emptyset$}
        \State $R \leftarrow
        R \cup
        \{\langle
        \widetilde{y}_1,\ldots,\widetilde{y}_c
        \rangle\}$
    \Else
        \State $R \leftarrow
        R \cup
        \{\langle
        g,
        \widetilde{y}_{1},
        \ldots,
        \widetilde{y}_{c}
        \rangle\}$
    \EndIf
\EndFor
\State \Return $R$
\Statex
\end{algorithmic}

\begin{algorithmic}[1]
\color{red}
\Statex \textbf{PAC-selection operator}
\[
\sigma^{\mathsf{pac}}_{\mathsf{p}}(T_1, T_2, \cdots, T_m)
\]
\vspace{0.25em}

\Statex \textbf{Input:}
$m$ input relations $T_1, T_2, \cdots, T_m$ that share the same schema.

\Statex \textbf{Output:}
$m$ output relations that share the same schema.
\vspace{0.25em}

\Return $\{\sigma_{\mathsf{p}}(T_1), \sigma_{\mathsf{p}}(T_2), \cdots, \sigma_{\mathsf{p}}(T_m)\}$
\Statex
\end{algorithmic}

\begin{algorithmic}[1]
\color{red}
\Statex \textbf{PAC-projection operator}
\[
\pi^{\mathsf{pac}}_{\mathsf{f}}(T_1, T_2, \cdots, T_m)
\]
\vspace{0.25em}

\Statex \textbf{Input:}
$m$ input relations $T_1, T_2, \cdots, T_m$ that share the same schema.

\Statex \textbf{Output:}
$m$ output relations that share the same schema.
\vspace{0.25em}

\Return $\{\pi_{\mathsf{f}}(T_1), \pi_{\mathsf{f}}(T_2), \cdots, \pi_{\mathsf{f}}(T_m)\}$
\Statex
\end{algorithmic}

\begin{algorithmic}[1]
\color{red}
\Statex \textbf{PAC-aggregation operator}
\[
\gamma^{\mathsf{pac}}_{G, \mathsf{Aggs}}(\mathcal{T})
\]
\vspace{0.25em}

\Statex \textbf{Input:}
A list of input relations $\mathcal{T}$, which contains either
(i) a single relation, or
(ii) $m$ relations sharing the same schema.

\Statex \textbf{Output:}
$m$ output relations that share the same schema.
\vspace{0.25em}

\If{$(|\mathcal{T}| = 1 \text{ and } \mathsf{pu} \notin \mathsf{Attr}(\mathcal{T}))$}
    \State \Return \textsf{undefined}
\EndIf

\If{$|\mathcal{T}| = m$}
    \State $\{T_1, \ldots, T_m\} \leftarrow \mathcal{T}$
    \State \Return 
    $\{T'_1 \gets \gamma_{G, \mathsf{Aggs}}(T_1), \ldots,
      T'_m \gets \gamma_{G, \mathsf{Aggs}}(T_m)\}$
\EndIf

\State $T'_1, \ldots, T'_m \leftarrow \emptyset$
%\State $\{\mathsf{Agg}_1(\alpha_1), \ldots, 
        %\mathsf{Agg}_c(\alpha_c)\} \leftarrow \mathsf{Aggs}$
\For {$i=1$ to $m$}
\State $\mathsf{sample}_i \leftarrow \sigma_{H(\mathsf{pu})[i]=1}(\mathcal{T})$
\State  $T'_i \leftarrow \gamma_{G, \mathsf{Aggs}}(\mathsf{sample}_i)$
\EndFor
\State \Return $\{T'_1, T'_2, \ldots, T'_m\}$
\Statex 
\end{algorithmic}



\begin{algorithmic}[1]
\color{red}
\Statex \textbf{PAC-join operator}
\[
\Join^{\mathsf{pac}}_{\theta}(\mathcal{T}_1, \mathcal{T}_2)
\]
\vspace{0.25em}

\Statex \textbf{Input:}
Two lists of input relations $\mathcal{T}_1$ and $\mathcal{T}_2$, where each list contains either
(i) a single relation, or
(ii) $m$ relations sharing the same schema.

\Statex \textbf{Output:}
$m$ output relations that share the same schema.
\vspace{0.25em}

\If{$(|\mathcal{T}_1| = 1 \text{ and } \mathsf{pu} \notin \mathsf{Attr}(\mathcal{T}_1))$ or $|\mathcal{T}_2| = 1 \text{ and } \mathsf{pu} \notin \mathsf{Attr}(\mathcal{T}_2))$}
    \State \Return \textsf{undefined}
\EndIf

\If {$|\mathcal{T}_1| = m$ }
\State $\{T_{1, 1}, \ldots, T_{1, m}\} \leftarrow \mathcal{T}_1$
\ElsIf {$|\mathcal{T}_1| = 1$ }
 \For {$i=1$ to $m$}
        \State $T_{1, i} \leftarrow \sigma_{H(\mathsf{pu})[i]=1}(\mathcal{T}_1)$
%        \State  $T'_i \gets \mathsf{sample}_i \Join_{\theta} T_{2, i}$
   \EndFor
\EndIf

\If {$|\mathcal{T}_2| = m$ }
\State $\{T_{2, 1}, \ldots, T_{2, m}\} \leftarrow \mathcal{T}_2$
\ElsIf {$|\mathcal{T}_2| = 1$ }
 \For {$i=1$ to $m$}
        \State $T_{2, i} \leftarrow \sigma_{H(\mathsf{pu})[i]=1}(\mathcal{T}_2)$
   \EndFor
\EndIf


\State \Return $\{T'_1 \gets T_{1, 1} \Join_{\theta} T_{2, 1}, \ldots,
      T'_m \gets T_{1, m} \Join_{\theta} T_{2, m}\}$
\end{algorithmic}
\end{multicols}
\hrulefill
\caption{Semantics of the PAC-relational-operators.}
\label{fig:pac-operators}
\end{figure*}



%\section{PAC-Private Semantics in Relational Algebra}

In this section, we introduce the semantics of PAC-private queries in the relational algebra setting.
We begin by defining the class of supported \emph{top queries}, denoted by $Q^{\mathsf{top}}(\mathcal{T})$.
Here, $\mathcal{T}$ denotes either one relation or $m$ relations
produced by a permitted subquery, denoted by $Q^{\mathsf{sub}}(\mathbb{I}, m)$. The subquery is evaluated over a list of permitted input base relations $\mathbb{I} = \{I_1, \ldots, I_n\}$ and a PAC privacy sampling parameter $m$.
We define the class of PAC-private queries $Q^{\mathsf{pac}}$ using the following grammar:
\[
Q^{\mathsf{pac}} ::= Q^{\mathsf{top}}\bigl(Q^{\mathsf{sub}}(\mathbb{I}, m)\bigr).
\]




In the remainder of this section, we first introduce the notations and assumptions used in our PAC-private relational algebra semantics. We then present the semantics of top queries $Q^{\mathsf{top}}(\mathcal{T})$, followed by the semantics of
subqueries $Q^{\mathsf{sub}}(\mathbb{I}, m)$. These semantics introduce PAC-private extensions of relational operators, covering the main mechanisms used in the original PAC database approach proposed in~\cite{}, as well as additional insights and refinements introduced in this work.

\subsection{Notations and Assumptions}
We denote by $\{0,1\}^l$ the set of all binary strings of length $l$, and by $[1,m]$ the set of integers from $1$ to $m$. 
The assignment $a \leftarrow b$ indicates that the value of $b$ is assigned to the variable $a$, while $a \stackrel{\$}{\leftarrow} C$ denotes that $a$ is sampled uniformly at random from the set $C$.  For a set or list $C$, we use $|C|$ to denote its cardinality. Given a set or bag of tuples $T$ whose schema consists only of the 
grouping attributes $G$ and the aggregation-result attributes $\mathsf{attr}_1, \mathsf{attr}_2, \ldots, \mathsf{attr}_c$, let $\mathsf{GAttr}(T) = (G, \mathsf{attr}_1, \mathsf{attr}_2, \ldots, \mathsf{attr}_c)$
denote this ordered list of attributes.
Given a relation $T$, let $\mathsf{Attr}(T)$ denote the set of
attributes in $T$. Given a relation $T$ that contains only grouping attributes
$G$ and aggregation-result attributes $\mathsf{attr}_1,\ldots,\mathsf{attr}_c$, we define $\mathsf{GAttr}(T) = (G,\mathsf{attr}_1,\ldots,\mathsf{attr}_c).$ Given $m$ aggregation results $y_1, y_2, \ldots, y_m$, let  $\mathsf{Var}_{\mathrm{emp}}(y_1, \ldots, y_m)$ outputs their empirical variance.
We adopt a hash function $H : \{0,1\}^* \rightarrow \{0,1\}^m$ that maps an arbitrary input value to a binary string of length $m$. 
For an input $x$, we write $H(x)[i]$ to denote the $i$-th bit of $H(x)$, for all $1 \leq i \leq m$.


In the semantics for PAC-private operators, we rely on standard (classical or extended) relational operators, including projection $\pi$, selection $\sigma$, natural join $\Join$, duplicate elimination $\delta$, intersection $\cap$, and union $\cup$.

We assume a single type of PU throughout the database, such as a user identifier, which is also a standard assumption in differentially private (DP) database systems~\cite{}. %Furthermore, we assume that each relation produced by the subquery $\mathcal{S}^{\mathsf{pac}}$—that is, each input relation to $\gamma^{\mathsf{pac}}_{G,\mathsf{Aggs}}$—contains at most one privacy-unit column $\mathsf{pu}$. As will be discussed in Section~\ref{sec:...}, this assumption implies that the subquery does not include join operations that would create shared ownership, i.e., tuples associated with more than one privacy-unit identifier. We emphasize that this restriction is introduced solely for clarity of presentation and does not represent an inherent limitation of PAC privacy.

\subsection{PAC-DB Semantics and Its Limitations}

In the seminal PAC-DB paper~\cite{cryptoeprint:2026/238}, each permitted SQL query $Q$—
typically an aggregation query at the top level—is treated as a black box.
To achieve PAC privacy, the framework generates $m$ independent samples
for each base relation used by $Q$, where each privacy-unit identifier
is included in each sample independently with probability $1/2$.
The query $Q$ is then evaluated over each sample,
producing $m$ query results.
For every group--aggregation cell that appears across the $m$ results,
the corresponding $m$ aggregation values are collected,
their empirical variance is computed,
and a noise distribution is calibrated accordingly.
One of the $m$ aggregation values is selected uniformly at random,
noise drawn from the calibrated distribution is added,
and the resulting value is released as the final output for that cell.

At first glance, representing this workflow in relational algebra
appears to require only two additional operators:
a sampling operator and a noise operator,
while the remaining computation could be expressed
using standard relational operators.
However, such a direct encoding merely captures
a syntactic decomposition of a PAC-private query $Q$
into query evaluation, sampling, and noising phases.
It does not expose structural opportunities for optimization,
particularly with respect to the dominant performance bottleneck
in PAC-DB—namely, executing the query over $m$ samples.

For example, if a sequence of relational operations
does not introduce shared ownership
(i.e., every tuple in the intermediate result
is associated with at most one privacy-unit identifier),
then sampling can be safely postponed
until a join or aggregation operator
where shared ownership may arise.
Deferring sampling in this manner
avoids redundant computation over $m$ samples
and can significantly improve efficiency.
Furthermore, standard relational operators are designed
to process one or two relations at a time,
and are therefore not well suited
to reasoning about or optimizing computations
that must be carried out simultaneously over $m$ samples.

To systematically capture these structural properties
and optimization opportunities,
we introduce dedicated PAC-private operators.
As will be shown in the following subsections,
a PAC-private query is represented
as a composition of standard relational operators
and PAC-specific operators,
thereby enabling both formal reasoning about privacy
and principled optimization at the relational-algebra level.
Our relational-algebra formulation provides three main advantages:

\begin{enumerate}
    \item \textbf{Deferred sampling.}
    Sampling of a base or intermediate relation
    is postponed until an operator that may introduce shared ownership,
    ensuring that sampling is performed only when necessary.

    \item \textbf{Hash-based sampling.}
    We adopt a hash-based sampling mechanism to simplify the sampling procedure.

    \item \textbf{PAC-specific multi-sample operators.}
    We introduce operators that operate directly over $m$ samples,
    enabling structured reasoning and optimization
    of computations that involve multiple samples.
\end{enumerate}



\subsection{PAC Relational Operators}
Our PAC-private relational algebra semantics introduces a set of dedicated PAC relational operators.
As illustrated in Figure~\ref{fig:pac-operators}, these include a PAC-noise operator
$\mathcal{N}^{\mathsf{pac}(\beta)}(T_1, \ldots, T_m)$,
a PAC-selection operator
$\sigma^{\mathsf{pac}}_{\mathsf{p}}(T_1, \ldots, T_m)$,
a PAC-projection operator
$\pi^{\mathsf{pac}}_{\mathsf{f}}(T_1, \ldots, T_m)$,
a PAC-aggregation operator
$\gamma^{\mathsf{pac}}_{G,\mathsf{Aggs}}(\mathcal{T})$,
and a PAC-join operator
$\Join^{\mathsf{pac}}_{\theta}(\mathcal{T}_1, \mathcal{T}_2)$.
Here, $m$ denotes the PAC sampling parameter.
Additional notation specific to each operator is introduced
when their semantics are defined.


\noindent (\textbf{PAC-noise operator.})
The legitimate input for the noise operator consists of a list of $m$ relations $\{T_1, \ldots, T_m\}$ that share the same schema. Each relation contains a (possibly empty) set of grouping attributes $G$ and a collection of aggregation-result attributes $\mathsf{attr}_1, \ldots, \mathsf{attr}_c$.
When the grouping attribute set $G$ is empty, each input relation contains exactly one tuple. 


In the case that $G$ is empty, the operator constructs a singleton group-value relation
$GV = \{\perp\}$, where $\perp$ denotes the unique (dummy) grouping value. Otherwise, when $G \neq \emptyset$, the operator constructs $GV$ to consist of all grouping values that appear in every one of the $m$ input relations.
For each group--aggregation cell defined by a pair $(g, \mathsf{attr}_j)$, where $g \in GV$ and
$1 \leq j \leq c$, the operator first computes the empirical variance $s^2_{j}$ over the $m$ aggregation values in the cell across the input relations. This empirical variance is then combined with the per-cell mutual-information budget $\beta$ to determine the variance
$\Delta_{j}$ of the Gaussian noise distribution.
Specifically, $\Delta_{j}$ is calibrated according to the
PAC-DB mechanism as a function of $s^2_{g,j}$ and $\beta$.
A Gaussian distribution $\mathcal{N}(0,\Delta_{j})$
is then constructed, from which a noise value is sampled.
One of the $m$ aggregation results is selected uniformly at random, and the sampled noise is added to this selected value. The resulting quantity constitutes the final noisy output for the corresponding group--aggregation cell.

If $G =\emptyset$, the output relation $R$ contains exactly one tuple where the $i$-th column stores the noised aggregation result for the cell of $(\perp, \mathsf{attr}_j)$. If $G =\neq$, each tuple in the output relation $R$ is constituted by a distinct grouping value $g \in GV$ and $c$ noised results, where the $i$-th noise result corresponds to the cell of $(g, \mathsf{attr}_j)$. 

\noindent (\textbf{PAC-selection and PAC-projection operators.})
A PAC-selection operator $\sigma^{\mathsf{pac}}_{\mathsf{p}}$
or PAC-projection operator $\pi^{\mathsf{pac}}_{\mathsf{f}}$
takes as input a list of $m$ relations
$\{T_1, \ldots, T_m\}$. The symbol $\mathsf{p}$ denotes an arbitrary predicate supported by
the standard selection operator $\sigma$, and $\mathsf{f}$ denotes an arbitrary expression supported by the standard projection operator $\pi$. The operator is applied independently to each input relation,
producing a corresponding output relation.
The overall result therefore consists of $m$ output relations, one for each input relation.

Importantly, PAC-selection and PAC-projection operate only
on already-sampled inputs. They do not perform the sampling step (i.e., they do not partition a relation into $m$ samples). This design reflects the fact that standard selection and projection can be safely applied to pre-sampling relations without introducing shared ownership.
By restricting sampling to operators where shared ownership may arise, we avoid unnecessary duplication of computation while preserving the intended PAC semantics.

%We allow selection and projection to be applied to the outputs of PAC-private aggregations because such operations may reduce the number of group-aggregation cells, thereby decreasing the overall privacy budget consumed by the query.
%where each privacy-unit identifier contributes independentlyto each relation with probability $1/2$.

\noindent (\textbf{PAC-aggregation operator.}) 
The input $\mathcal{T}$ to $\gamma^{\mathsf{pac}}_{G,\mathsf{Aggs}}$ consists either of a single relation or of $m$ relations.
A single input relation indicates that sampling has not yet been performed and that all preceding operators preserve the
single-owner property (i.e., no shared ownership has been introduced).
Here, $G$ denotes the set of grouping attributes, and $\mathsf{Aggs}$ represents a list of aggregation operations over
aggregation attributes:$\mathsf{Aggs}=\{\mathsf{Agg}_1(\alpha_1), \mathsf{Agg}_2(\alpha_2), \ldots, \mathsf{Agg}_c(\alpha_c)\}.$


If $\mathcal{T} = \{T_1, \ldots, T_m\}$,
the operator applies the standard aggregation independently
to each relation and produces $m$ output relations: $T'_i=\gamma_{G,\mathsf{Aggs}}(T_i),$ for all $1 \le i \le m$. In this case, no additional sampling is performed, since the sampling semantics have already been established upstream.


If $\mathcal{T}$ consists of a single relation $T$, its schema must include the privacy-unit attribute $\mathsf{pu}$
that identifies the owner of each tuple; otherwise, the operator is undefined.
In this setting, the operator conceptually generates $m$ independent samples of $T$,
such that each privacy-unit identifier is included in each sample independently with probability $1/2$.
The standard aggregation operator is then applied to each sample, producing $m$ output relations.

To realize this sampling semantics efficiently, we adopt a hash-based approach: a privacy-unit identifier $\mathsf{pu}$ is included
in the $i$-th sample if and only if $H(\mathsf{pu})[i] = 1$, where $H: \{0,1\}^* \to \{0,1\}^m$ is assumed to be a uniformly random hash function. Under this assumption, each privacy unit is included in each sample independently with probability $1/2$.

\textbf{Optimization.} Section~\ref{sec:...} describes an optimized implementation of this operator using SIMD-based techniques when the aggregation function is 
incremental.

\noindent (\textbf{PAC-join operator.}) The PAC-join operator $\Join^{\mathsf{pac}}_{\theta}$ takes as input two collections of relations, denoted by $\mathcal{T}_1$ and $\mathcal{T}_2$. Each collection contains either a single relation or $m$ relations. Similar to the PAC-aggregation operator, the PAC-join operator is invoked only when a join operation may introduce shared ownership in the output tuples. In particular, it is used in cases where joining the inputs could associate a resulting tuple with multiple privacy-unit identifiers, thereby requiring PAC sampling semantics. Therefore, if  




%Moreover, when 
%$\gamma^{\mathsf{pac}}_{G,\mathsf{Aggs}}(\mathcal{T})$ %appears in a 
%top-level query, the privacy-unit attribute $\mathsf{pu}$ must not be 
%included among the grouping attributes $G$. 
%Otherwise, the released output would directly reveal whether a  particular privacy unit contributed to the result, giving the adversary  a posterior advantage of~1.




\subsection{Semantics for Top Queries}

To define the semantics of top queries $Q^{\mathsf{top}}$, we introduce four PAC-private extended operators: a PAC-private aggregation operator, a PAC-private selection operator, a PAC-private projection operator, and a PAC-private noise operator. 

Let $\mathcal{T}$ be the output of $Q^{\mathsf{sub}}(\mathbb{I}, m)$, whose semantics will be defined
in the following subsection. The class of PAC-private top queries is defined by the grammar
\[
Q^{\mathsf{top}} ::=
\mathcal{N}^{\mathsf{pac}(\beta)}
\Bigl(
\pi^{\mathsf{pac}}_{\widehat{G},\widehat{\mathsf{f}}}
\sigma^{\mathsf{pac}}_{\mathsf{p}}
\gamma^{\mathsf{pac}}_{\widehat{G},\mathsf{Aggs}}
(\mathcal{T})
\Bigr),
\]
subject to the following well-formedness conditions:
\begin{itemize}
    \item[(i)] The grouping attribute set $\widehat{G}$ must not contain
    the privacy-unit attribute.
    \item[(ii)] The operators
    $\pi^{\mathsf{pac}}$ and
    $\sigma^{\mathsf{pac}}$ are optional,
    whereas the aggregation and noise operators are mandatory.
    \item[(iii)] The projection expression
    $\widehat{\mathsf{f}}$ may involve only aggregation-result
    attributes.
    \item[(iv)] If $\pi^{\mathsf{pac}}$ is present and
    $\widehat{G}\neq\emptyset$, then all attributes in
    $\widehat{G}$ must be included in the projection before the
    noise operator is applied.
\end{itemize}

Intuitively, the subquery $Q^{\mathsf{sub}}$ produces a collection of intermediate relations $\mathcal{T}$, where
$|\mathcal{T}|$ is either $1$ or $m$, depending on whether the subquery produces shared ownership or not.
The operator $\gamma^{\mathsf{pac}}_{\widehat{G},\mathsf{Aggs}}$ then performs a PAC-private aggregation, producing $m$ output
relations. The operators $\sigma^{\mathsf{pac}}_{\mathsf{p}}$ and $\pi^{\mathsf{pac}}_{\widehat{G},\widehat{\mathsf{f}}}$
subsequently apply selection and projection to the aggregation outputs.
Finally, the noise operator $\mathcal{N}^{\mathsf{pac}(\beta)}$ injects PAC-calibrated noise into the aggregation results,
ensuring that each output cell—defined by a distinct value of the grouping attributes $\widehat{G}$ and each aggregation function
after selection and projection—satisfies the privacy budget $\beta$.

When 
$\gamma^{\mathsf{pac}}_{G,\mathsf{Aggs}}(\mathcal{T})$ appears in a  top-level query, the privacy-unit attribute $\mathsf{pu}$ must not be 
included among the grouping attributes $G$. 
Otherwise, the released output would directly reveal whether a  particular privacy unit contributed to the result, giving the adversary 
a posterior advantage of~1.


We allow selection and projection to be applied to the outputs of PAC-private aggregations because such operations may reduce the number of group-aggregation cells, thereby decreasing the overall privacy budget consumed by the query.




\begin{table*}[t]
\centering
\caption{Allowed Operators for Single-owner Subqueries $\mathcal{S}^{\mathsf{single}}$}
\label{tab:allowed-singlesubquery-operators}
\small
\color{red}
\begin{tabular}{llll}
\toprule
\textbf{Operator} & \textbf{Allowed Form} & \textbf{Schema Constraints} & \textbf{Notation}\\
\midrule

\multirow{2}{*}{Projection $\pi$}
& $\pi_{\mathsf{pu}, \mathbf{f}}(T)$
& $\mathsf{pu} \in \mathsf{Attr}(T)$
& \multirow{2}{*}{$\mathbf{f}$ denotes standard projection expressions that do not involve $\mathsf{pu}$.}\\[0.3em]
& $\pi_{\mathbf{f}}(T)$
& $\mathsf{pu} \notin \mathsf{Attr}(T)$
& \\

\midrule
Selection $\sigma$
& $\sigma_{\mathbf{p}}(T)$
& none
& $\mathbf{p}$ denotes standard selection predicates. \\

\midrule
\multirow{2}{*}{Aggregation $\gamma$}
& $\gamma_{\{\mathsf{pu}\} \cup G, \mathsf{Aggs}}(T)$
& $\mathsf{pu} \in \mathsf{Attr}(T)$
& \multirow{2}{*}{$G$ denotes grouping attributes that do not involve $\mathsf{pu}$.}\\[0.3em]
& $\gamma_{G, \mathsf{Aggs}}(T)$
& $\mathsf{pu} \notin \mathsf{Attr}(T)$
& \\

\midrule
\multirow{2}{*}{Join $\Join$}
& $T_1 \Join_{(T_1.\mathsf{pu} = T_2.\mathsf{pu}) \wedge \theta} T_2$
& $\mathsf{pu} \in \mathsf{Attr}(T_1)$ and $\mathsf{pu} \in \mathsf{Attr}(T_2)$
& \multirow{2}{*}{$\theta$ denotes standard join predicates that do not involve $\mathsf{pu}$.}\\[0.4em]
& $T_1 \Join_{\theta} T_2$
& $\mathsf{pu} \notin \mathsf{Attr}(T_1)$ or $\mathsf{pu} \notin \mathsf{Attr}(T_2)$
& \\

\bottomrule
\end{tabular}
\end{table*}

\subsection{Semantics for Subqueries}

The supported subqueries are divided into two subclasses.
The first subclass consists of subqueries in which each generated
tuple is associated with exactly one privacy-unit identifier.
Such subqueries can be expressed using standard relational algebra,
under the restriction that no shared ownership is introduced during
their evaluation.
The second subclass captures cases in which tuples may be associated
with multiple privacy-unit identifiers, resulting in shared ownership.
These subqueries require the use of the PAC-private relational
operators introduced in the previous subsection, as well as
additional operators defined in this subsection.

We refer to the first subclass as
\emph{single-owner subqueries},
denoted by
$\mathcal{S}^{\mathsf{single}}(\cdot)$, which takes as input a set (or subset) of base relations and output an output relation. We refer to the second subclass as
\emph{shared-owner subqueries},
denoted by
$\mathcal{S}^{\mathsf{shared}}(\cdot)$. Intuitively, a shared-owner subquery is constructed from the
outputs of several single-owner subqueries together with
additional base relations, which may introduce shared ownership. A permitted subquery $Q^{\mathsf{sub}}(\mathbb{I},m)$ may belong to either subclass.
Formally, we define
\[
Q^{\mathsf{sub}}(\mathbb{I},m)
::=
\mathcal{S}^{\mathsf{single}}(\mathbb{I})
\;\; \mid \;\;
\mathcal{S}^{\mathsf{shared}}
\bigl(
\mathbb{V} \cup
\mathbb{I}^{\iota+1},\,
m
\bigr),
\]
where
\[
\mathbb{V}
=
\{V_1,\ldots,V_{\iota}\},
\quad
V_i ::= \mathcal{S}^{\mathsf{single}}(\mathbb{I}^i),
\]
and the following conditions hold: (i) $\iota \ge 0$; (ii) $\mathbb{I}^i \subseteq \mathbb{I}$ for all $1 \le i \le \iota+1$; (iii) the subsets are pairwise disjoint, i.e., $\mathbb{I}^i \cap \mathbb{I}^j = \emptyset$ for all $1 \le i < j \le \iota+1$, and (iv) they form a partition of $\mathbb{I}$, i.e. $\mathbb{I}^1 \cup \cdots \cup \mathbb{I}^{\iota+1} = \mathbb{I}.$


%Let $T_1$ be an output relation of $\mathcal{S}^{\mathsf{single}}(\mathbb{I}, m)$. We refer to the second subclass as \emph{shared-owner subqueries}, denoted by $\mathcal{S}^{\mathsf{shared}}(T)$. 

%The class of PAC-private subqueries is defined by the grammar $$Q^{\mathsf{sub}}::==$$

 

\subsubsection{Base Relations $\mathbb{I}$}
Let $I \in \mathbb{I}$ be a base relation. We assume that a base relation $I$ may or may not be contributed by privacy units. If a base relation $I$ is contributed by privacy units, we assume that each tuple in $I_i$ is associated with exactly one privacy-unit identifier, and that a privacy-unit attribute $\mathsf{pu}$ is included in the schema of $I_i$ to indicate the owner of each tuple.

In practice, even when $I_i$ is contributed by privacy units, the relation may not explicitly contain the $\mathsf{pu}$ attribute. To address this issue, Section~\ref{sec:...} describes an automatic join mechanism that ensures the inclusion of the $\mathsf{pu}$ attribute whenever a privacy-unit–contributed relation is used as a base input to a PAC-private query. In this subsection, for clarity of presentation, we assume that this automatic join has already been applied before executing any subquery
$\mathcal{S}^{\mathsf{single}}$ or $\mathcal{S}^{\mathsf{shared}}$.
  

\subsubsection{Single-owner Subqueries} 
A single-owner subquery $\mathcal{S}^{\mathsf{single}}$
is defined as a relational algebra expression whose operator nodes
are drawn from the set of allowed operators specified in
Table~\ref{tab:allowed-singlesubquery-operators}.
In particular, $\mathcal{S}^{\mathsf{single}}$ is constructed using
standard relational operators—projection ($\pi$),
selection ($\sigma$), aggregation ($\gamma$), and join ($\Join$)—
subject to the restricted forms described in the table.
single-owner subqueries are closely related to the class of
subqueries used in differentially private query processing
frameworks, as described in~\cite{}.
The main difference is that our formulation explicitly supports
relations both with and without $\mathsf{pu}$ contributions,
whereas prior semantics typically assume that all relations
contain a $\mathsf{pu}$ attribute.


The key invariant of a single-owner subquery is that no shared
ownership is introduced during evaluation.
More precisely, for every base, intermediate, or final relation $T$
that contains tuples contributed by privacy units,
the following conditions must hold:
(i) each tuple in $T$ is associated with exactly one privacy-unit
identifier; and
(ii) the attribute $\mathsf{pu}$ appears in the schema of $T$
to explicitly indicate ownership.

For relations $T$ that do not involve privacy-unit contributions,
no additional restrictions are imposed.
For relations that do contain $\mathsf{pu}$, the operators must
preserve the single-owner property as follows. 

\textbf{Projection.}
If $T$ contains $\mathsf{pu}$, then $\mathsf{pu}$ must be included
in the projection list.
Moreover, $\mathsf{pu}$ may not be used to derive other attributes,
as this could implicitly introduce untracked shared ownership.

\textbf{Aggregation.}
Aggregation can potentially merge tuples contributed by different
privacy units.
To prevent shared ownership, whenever $T$ contains $\mathsf{pu}$,
the attribute $\mathsf{pu}$ must be included among the grouping
attributes of the aggregation operator.

\textbf{Join.}
A join may introduce shared ownership when both input relations
contain tuples contributed by privacy units.
To preserve the single-owner property, if both inputs contain
$\mathsf{pu}$, the join condition must enforce equality of the
privacy-unit identifiers, i.e., tuples may only join when they
share the same $\mathsf{pu}$ value.
If at least one input relation does not contain $\mathsf{pu}$,
then no shared ownership can arise from the join,
and arbitrary join predicates are permitted.

\textbf{Selection.}
The selection operator does not affect ownership, as it only filters tuples without altering their contributors.
Therefore, no additional restrictions are required for $\sigma$.     


\subsubsection{Shared-owner Subqueries}

To define shared-owner subqueries, denoted by
$\mathcal{S}^{\mathsf{shared}}$, we introduce a PAC-private join operator
$\Join^{\mathsf{pac}}$, whose semantics are given in
Figure~\ref{fig:pac-private-join}.

A shared-owner subquery $\mathcal{S}^{\mathsf{shared}}$ is defined as a
relational algebra expression whose operator nodes are drawn from the
set of PAC-private operators
\[
\{\gamma^{\mathsf{pac}},\; \sigma^{\mathsf{pac}},\; \pi^{\mathsf{pac}},\; \Join^{\mathsf{pac}}\}.
\]
Such expressions must satisfy the following structural constraint:
every leaf-level operator in the relational algebra tree—namely, every
operator whose inputs are base relations or outputs of single-owner
subqueries—must be either $\gamma^{\mathsf{pac}}$ or
$\Join^{\mathsf{pac}}$.

This constraint ensures that PAC sampling is introduced only at points where shared ownership may arise. All operations that occur prior to the introduction of shared ownership are handled within single-owner subqueries. By deferring sampling in this manner, we avoid applying operators over $m$ samples unnecessarily, thereby reducing performance overhead while preserving the intended ownership semantics.
\color{black}

\subsection{Algebraic Query Translation}
We apply PAC as late as possible!
\label{sec:translation}


\subsection{Equivalence of Optimized and Naïve PAC}
\begin{itemize}
  \item Per-sample invariants
  \item Order independence
  \item Formal equivalence argument
  \item Closure under post processing
\end{itemize}

%In this subsection, we characterize the class of permitted subqueries $\mathcal{S}$ and the corresponding levels of PAC privacy guarantees they provide. We begin with \emph{subqueries without cross-pu aggregations}, namely subqueries that do not invoke the PAC-private aggregation operator $\digamma$. We denote this class by $\mathcal{S}^0$. We subsequently consider subqueries that contain $\digamma$ and therefore consume positive privacy budget, denoted by $\mathcal{S}^{+}$.

%\textbf{\textit{Base Relations.}}
%Let $I_i$ be a base relation for $1 \leq i \leq \iota$. We assume that each base relation contains at most one privacy unit attribute. When present, for ease of exposition, we denote this attribute by $\mathsf{pu}\!\parallel\!1$. Moreover, we assume that any relation contributed by privacy units must include its privacy unit attribute in its schema.

%\textbf{\textit{Subqueries without cross-pu aggregation.}} The relational operators permitted in $\mathcal{S}^0$ are summarized in Table~\ref{tab:allowed-subquerys0-operators}. We use $T_s$, $T_{s1}$, and $T_{s2}$ to denote the input relations to each operator. The allowed operators include projection ($\pi$), selection ($\sigma$), aggregation ($\gamma$), and join ($\Join$).

%For projection, if the input relation $T_s$ contains privacy unit attributes, all such attributes must be preserved in the projection to ensure that tuple ownership can be tracked. Additional projected expressions $\mathbf{f}$ are permitted provided that they do not reference privacy unit attributes. If $T_s$ contains no privacy unit attributes, an arbitrary projection $\pi_{\mathbf{f}}(T_s)$ is allowed. For selection, arbitrary Boolean predicates $\mathbf{p}$ that do not reference privacy unit attributes are permitted. For aggregation, if $T_s$ contains privacy unit attributes, all such attributes must be included in the grouping key, together with any additional grouping attributes $\mathsf{ga}$ that exclude privacy unit attributes. Standard aggregation functions are then applied. This restriction ensures that aggregation does not introduce shared ownership. If $T_s$ contains no privacy unit attributes, conventional aggregation is allowed.

%Shared ownership may only arise through join operations.For joins with predicate $\theta$ that does not reference privacy unit attributes, privacy unit attributes in $T_{s2}$ are renamed. Specifically, each attribute $\mathsf{pu}\!\parallel\!i$ in $T_{s2}$ is renamed to $\mathsf{pu}\!\parallel\!(\eta_1+i)$, where $\eta_1$ is the number of privacy unit attributes in $T_{s1}$. When $\Lambda(\mathsf{schema}(T_{s2})) = 0$, no renaming of privacy unit attributes is required. We additionally allow join predicates that are conjunctions of equality conditions over privacy unit attributes.

%\begin{theorem}
%Let $\{I_1, \ldots, I_{\iota}\}$ be a collection of base relations, where each base relation $I_i$, for $1 \leq i \leq \iota$, contains at most one privacy unit attribute, denoted by $\mathsf{pu}\!\parallel\!1$. Let $T \leftarrow \mathcal{S}^0(I_1, \ldots, I_{\iota})$ be the result of a subquery that can be represented by a relational algebra tree whose operators are drawn from Table~\ref{tab:allowed-subquerys0-operators}. Let $\mathsf{ga}$ be a set of grouping attributes that contains no privacy unit attribute, and let $\{\mathsf{PAgg}_1(\alpha_1), \ldots, \mathsf{PAgg}_c(\alpha_c)\}$ be a sequence of $c$ PAC-private aggregation functions and their corresponding aggregation variables. Then the output of the PAC-private relational aggregation operator
%\[\digamma_{\mathsf{ga},\,\mathsf{PAgg}_1(\alpha_1),\ldots,\mathsf{PAgg}_c(\alpha_c)}^{(\mathsf{pu},\,\beta)}(\mathsf{PU}, T)\]
%satisfies PAC privacy with mutual information budget $t\beta$ with respect to the privacy unit $\mathsf{pu}$, where $t$ denotes the total number of group--aggregation cells induced by the grouping attributes $\mathsf{ga}$..
%\end{theorem}
%\begin{proof}

%\end{proof}


%\color{black}

%This is a difference from the PAC-DB mecahnism, where they only perform sampling over base relations. Their sampling approach constructs a table \textsf{PU} that lists all the privacy unit identifiers, and conduct possion sampling to create $m$  \textsf{PU} samples with the guarantee that each privacy-unit identifier is included in the each \txetsf{PU} sample with probability $1/2$, and join each \txetsf{PU} sample with the base relation on the privacy unit attribute to obtain $m$ samples for the base relation. Therefore, it can be seen that for sampling, we have two improvements: we allow sampling on intermediate relations without shared ownership, and we use hash-based sampling to avoid the join operations used in the PAC-DB approach.   

==> sections/pacra_2.tex <==
% Requires in preamble:
%   \newtheorem{lemma}{Lemma}[section]
%   \newtheorem{theorem}{Theorem}[section]
%   \newtheorem{definition}{Definition}[section]

\section{PAC Relational Algebra}
\label{sec:algebra}

\color{blue}
In this section, we formalize the query compilation approach of our
PAC-privatized query engine, proving the equivalence of our single-query bitslice rewrite and PAC-DB's multi-execution approach in Section.

\subsection{PAC-DB Semantics}
\label{sec:pacdb-semantics}
\vspace*{0mm}\noindent{\bf Notation.}
Let $U$ denote the designated privacy unit (PU) table with primary key attribute~$\mathsf{pk}_U$.
A base relation~$T$ may be linked to~$U$ through a foreign key chain $T \xrightarrow{fk_1} T_1 \xrightarrow{fk_2} \cdots \xrightarrow{fk_k} U$;
each tuple $t \in T$ is then associated with exactly one PU identifier, which we denote $\mathsf{pu}(t)$, obtained by following the foreign key path.
We write $m$ for the number of subsamples in our approach ($m{=}64$) and $\beta$ for the per-cell mutual information (MI) budget.
We adopt a hash function $H : \mathrm{dom} \to \{0,1\}^m$
and write $H(x)[j]$ for the $j$-th bit of $H(x)$, where $1 \le j \le m$. Further, given $m$ values $y_1, \ldots, y_m$, we write
$\mathsf{Var}_{\mathrm{emp}}(y_1, \ldots, y_m)
= \frac{1}{m-1}\sum_{i=1}^{m}(y_i - \bar{y})^2$
for their empirical variance, and $k \xleftarrow{\$} [1,m]$ for uniform random selection. 

\vspace*{0mm}\noindent{\bf Sampling.}
PAC-DB~\cite{sridhar2026pacdb} privatizes a query $Q$ by generating
$N$ independent subsamples of the PU population ($N{=}128$ in PAC-DB).
Each PU identifier $u \in U$ is included in subsample~$j$ independently with probability $\frac{1}{2}$, yielding subsamples
$S_1, \ldots, S_N \subseteq U$.
For dependent tables $T$ linked to $U$ through foreign keys, the subsample
propagates:
$S_j(T) = \{t \in T : \mathsf{pu}(t) \in S_j\}$.
The query $Q$ is then evaluated independently on each subsample, producing
$N$ results $Q(S_1), \ldots, Q(S_N)$.
The full PAC-DB execution reads
\begin{equation}\label{eq:pacdb}
\mathsf{PAC\text{-}DB}(Q)
= \mathcal{N}^{\mathsf{pac}(\beta)}\!\bigl(
  Q(S_1(T)),\;\ldots,\;Q(S_N(T))
\bigr),
\end{equation}
where $\mathcal{N}^{\mathsf{pac}(\beta)}$ denotes the noise mechanism
described next.

In our approach, we replace the $N$ independent random subsamples with $m{=}64$ hash-derived subsamples, defining the subsample operator
$\mathcal{S}_j(T) = \sigma_{H(\mathsf{pu}(t))[j]=1}(T)$
for $j \in [1, m]$.
The reduction from $N{=}128$ to $m{=}64$ subsamples is justified by a security analysis presented in Section~\ref{sec:hash-proof}.

\vspace*{0mm}\noindent{\bf Noise mechanism $\mathcal{N}^{\mathsf{pac}(\beta)}$.} [todo replace with p variance?]
Given $m$ subsample results $y_{1,i}, \ldots, y_{m,i}$ for a
group-aggregation cell $(g, \mathsf{attr}_i)$, the mechanism computes
the empirical variance
$s_i^2 = \mathsf{Var}_{\mathrm{emp}}(y_{1,i}, \ldots, y_{m,i})$,
calibrates the noise variance as
$\Delta_i = s_i^2 / (2\beta)$,
selects a subsample index $k \xleftarrow{\$} [1, m]$,
and releases the noised value
$\tilde{y}_i = y_{k,i} + \mathcal{N}(0, \Delta_i)$.
This ensures that the MI between the secret subsample identity and the released value satisfies
$I(S;\, \tilde{y}) \le \beta$ per cell~\cite{sridhar2025pac}.
%The cost of the PAC-DB approach is $N$ independent query executions, each joined with a sample table of size $|U|$.
%Our compiler eliminates both the multi-fold execution and the explicit sample-table joins.


%% ----------------------------------------------------------------
\subsection{PAC Functions}
\label{sec:pac-functions}
PAC functions evaluate all $m$ subsamples simultaneously within a
single query execution by exploiting the bitwise structure of the hash.

\vspace*{0mm}\noindent{\bf Bitslice counter aggregate
($\mathsf{pac\_agg\_ctr}$).} \\
For $\mathsf{agg} \in \{\mathsf{sum}, \mathsf{count}, \mathsf{avg},
\mathsf{min}, \mathsf{max}\}$,
the bitslice counter aggregate
$\mathsf{pac\_agg\_ctr}(h, e)$
takes a PU hash value $h = H(\mathsf{pu}(t)) \in \{0,1\}^m$
and an expression~$e$, and returns a vector of $m$ counters
$\mathbf{c} = \langle c_1, \ldots, c_m \rangle$ defined by
\begin{equation}\label{eq:counter}
c_j \;=\;
\mathsf{agg}\!\bigl(\{e(t) : t \in T \;\land\; H(\mathsf{pu}(t))[j] = 1\}\bigr),
\quad j = 1, \ldots, m.
\end{equation}
Each counter independently accumulates contributions from tuples whose PU hash has the corresponding bit set. A single evaluation of $\mathsf{pac\_agg\_ctr}$ therefore simultaneously
computes the aggregate results for all $m$ subsamples through bit-parallel operations on the hash.

\vspace*{0mm}\noindent{\bf Fused aggregate ($\mathsf{pac\_agg}$).}
The fused variant combines counter computation with noise application:
\begin{equation}\label{eq:fused}
\mathsf{pac\_agg}(h, e)
\;\equiv\;
\mathsf{pac\_noised}\!\bigl(\mathsf{pac\_agg\_ctr}(h, e)\bigr),
\end{equation}
returning a single noised scalar rather than the full counter vector.
The fused form applies whenever the aggregate result appears directly
in the query output and no downstream operator --- such as a comparison,
filter, or arithmetic expression --- requires access to individual
per-subsample values.
Conversely, $\mathsf{pac\_agg\_ctr}$ is required when the aggregate
feeds into a \emph{categorical context} (defined below), where each
subsample's outcome must be evaluated independently before a terminal noise or filter function can be applied.

\vspace*{0mm}\noindent{\bf Noise function ($\mathsf{pac\_noised}$).}
The scalar function $\mathsf{pac\_noised}(\mathbf{c})$
takes a counter vector $\mathbf{c} = \langle c_1, \ldots, c_m \rangle$
and applies the PAC-DB noise mechanism~$\mathcal{N}^{\mathsf{pac}(\beta)}$:
it computes $s^2 = \mathsf{Var}_{\mathrm{emp}}(\mathbf{c})$,
sets $\Delta = s^2 / (2\beta)$,
selects $k \xleftarrow{\$} [1, m]$,
and returns $c_k + \mathcal{N}(0, \Delta)$.

\vspace*{0mm}\noindent{\bf Categorical functions.} [todo- is this the final version?]
When the result of a PAC aggregate participates in a comparison or filter expression --- a \emph{categorical context}, e.\g. TPC-H Q?? --- noise cannot be applied at the
aggregate level.
The fundamental issue is that subsampling and filtering do not commute
when the filter depends on an aggregate result: evaluating a filter on a
subsampled aggregate may yield different outcomes than subsampling the
result of the filter applied to the full data.
To handle this, the aggregate must return the full counter vector,
and the categorical decision is deferred until all $m$ outcomes are available.

The function $\mathsf{pac\_filter}(\mathbf{b})$,
where $\mathbf{b} \in \{0,1\}^m$ is a vector of boolean outcomes
across the $m$ subsamples, produces a single probabilistic boolean:
\begin{equation}\label{eq:pac-filter}
P\!\bigl(\mathsf{pac\_filter}(\mathbf{b}) = \mathsf{true}\bigr)
\;=\;
\frac{\mathrm{popcount}(\mathbf{b})}{m}.
\end{equation}

This function applies at the outermost filter level, specifically when no PAC aggregate appears above the filter in the query plan. The fused variant
$\mathsf{pac\_filter\_cmp}(v, \mathbf{c})$
for $\mathsf{cmp} \in \{>, <, \ge, \le, =\}$
combines comparison and filtering: it evaluates
$b_j = \mathbb{1}[v \;\mathsf{cmp}\; c_j]$
for each $j$ and returns $\mathsf{pac\_filter}(\mathbf{b})$.
Algebraic simplification may absorb constant arithmetic into the
scalar argument (e.g., the predicate $x < 0.2 \cdot c$ is equivalently expressed as
$\mathsf{pac\_filter\_lt}(5x, \mathbf{c})$).

When a categorical filter sits \emph{below} an outer PAC aggregate,
a single boolean decision would destroy per-subsample information
needed by that aggregate.
The function $\mathsf{pac\_select}(h, \mathbf{b})$
computes the bitwise intersection
\begin{equation}\label{eq:pac-select}
\mathsf{pac\_select}(h, \mathbf{b}) \;=\; h \;\mathsf{AND}\; \mathbf{b},
\end{equation}
producing a \emph{reduced hash} in which bit~$j$ is~1 only if the tuple belongs to subsample~$j$ \emph{and} the condition holds in that subsample. The outer aggregate receives this reduced hash as its first argument, so its counter~$j$ accumulates only tuples that both belong to $S_j$ and pass the filter within~$S_j$. 
% This is equivalent to PAC-DB's behavior: PAC-DB selects
% $k \xleftarrow{\$} [1,m]$ and returns $b_k$;
% since $k$ is uniform,
% $P(b_k{=}1) = \frac{1}{m}\sum_j b_j
% = \mathrm{popcount}(\mathbf{b})/m$,
% which matches Equation~\ref{eq:pac-filter}.



%% ----------------------------------------------------------------
\subsection{Translation Rules}
\label{sec:translation-rules}

The compiler transforms a standard query plan~$Q$ into a
privacy-augmented plan~$\widehat{Q}$ through the translation rules
described below.
% A query is eligible for compilation if it contains at least one aggregation over PU-linked data, does not return protected columns outside an aggregate, and joins PU-linked tables exclusively over the registered PAC links (supporting inner, semi-, anti-, and outer join forms). The compiler rejects queries that would expose protected data and passes through queries that do not reference PU-linked tables.
Throughout the translation, a key invariant---the \emph{single-owner property} --- must hold for all intermediate relations prior to the PAC aggregation: every tuple is associated with at most one PU identifier. Standard selections and projections preserve this property; joins between two PU-linked relations preserve it only when the join equates their PU identifiers; and sub-aggregations preserve it only when the PU attribute is included in the grouping key.

\vspace*{0mm}\noindent{\bf PU join addition.}
When the query scans a table~$T$ linked to PU table~$U$ via the foreign key
chain $T \xrightarrow{fk_1} T_1 \xrightarrow{fk_2} \cdots
\xrightarrow{fk_k} U$
and the plan does not already contain a join path from~$T$ to~$U$,
the compiler inserts the missing intermediate joins.
Each added scan projects only the primary and foreign key columns
necessary for hash derivation, minimizing the data footprint:
\begin{equation}\label{eq:join-addition}
\mathrm{Scan}(T)
\;\longmapsto\;
\mathrm{Scan}(T)
\;\bowtie_{fk_1}\;
\pi_{\mathsf{pk}_1,\,fk_2}\!\bigl(\mathrm{Scan}(T_1)\bigr)
\;\bowtie_{fk_2}\;
\cdots
\end{equation}
When $U$ is already scanned in the original plan, no joins are added.

\vspace*{0mm}\noindent{\bf Join elimination.} 
Let $T_k$ be the last intermediate table before~$U$ in the foreign key path, with column $T_k.fk_U$ referencing $U.\mathsf{pk}$.
By referential integrity, $T_k.fk_U = U.\mathsf{pk}$ for every matching tuple, so the hash computed from the FK column is identical to the hash from the PK:
\begin{equation}\label{eq:join-elim}
H(T_k.fk_U) = H(U.\mathsf{pk})
\quad\text{for all matching tuples.}
\end{equation}
For composite PU keys $(k_1, \ldots, k_n)$, the hash input is formed as $k_1 \oplus \cdots \oplus k_n$ where~$\oplus$ denotes bitwise XOR.

\vspace*{0mm}\noindent{\bf Aggregate replacement.}
Every aggregation $\gamma_{G,\,\mathsf{agg}(e)}$ operating on PU-linked
tuples is rewritten to its PAC equivalent.
The compiler determines the hash expression~$h$ from the join addition
or elimination step and selects the appropriate variant.
In the non-categorical case, the fused variant is used:
\begin{equation}\label{eq:agg-fused}
\gamma_{G,\,\mathsf{agg}(e)}(T)
\;\longmapsto\;
\gamma_{G,\,\mathsf{pac\_agg}(h,\,e)}(T).
\end{equation}
When the aggregate result participates in a downstream comparison,
filter, or arithmetic expression that requires per-subsample evaluation,
the counter variant is used:
\begin{equation}\label{eq:agg-counter}
\gamma_{G,\,\mathsf{agg}(e)}(T)
\;\longmapsto\;
\gamma_{G,\,\mathsf{pac\_agg\_ctr}(h,\,e)}(T).
\end{equation}

\vspace*{0mm}\noindent{\bf Categorical expression rewrite.}
When an expression~$\phi$ in a selection, projection, join, or top-$k$
references a $\mathsf{pac\_agg\_ctr}$ result, it must be evaluated
\emph{elementwise} across all $m$ positions.
For a single counter vector~$\mathbf{c}$, the expression is lifted to
\begin{equation}\label{eq:categorical-single}
\phi[\mathbf{c}]
\;\longmapsto\;
\bigl\langle
\phi(c_1),\;\phi(c_2),\;\ldots,\;\phi(c_m)
\bigr\rangle.
\end{equation}
When~$\phi$ references multiple counter vectors
$\mathbf{c}^{(1)}, \ldots, \mathbf{c}^{(n)}$
(e.g., an arithmetic expression involving two PAC aggregates),
the vectors are combined position-wise:
\begin{equation}\label{eq:categorical-multi}
\phi\!\bigl[\mathbf{c}^{(1)}, \ldots, \mathbf{c}^{(n)}\bigr]
\;\longmapsto\;
\Bigl\langle
\phi\!\bigl(c_1^{(1)}, \ldots, c_1^{(n)}\bigr),\;\ldots,\;
\phi\!\bigl(c_m^{(1)}, \ldots, c_m^{(n)}\bigr)
\Bigr\rangle.
\end{equation}
The resulting vector~$\mathbf{r}$ is then wrapped by a terminal function that depends on the operator context.
In a projection or sort, $\mathsf{pac\_noised}(\mathbf{r})$ produces a noised scalar for output.
In a filter without an outer PAC aggregate,
$\mathsf{pac\_filter}(\mathbf{r})$ produces a probabilistic boolean.
In a filter \emph{with} an outer aggregate, the original join or semi-join is replaced by a cross product, a projection computes the reduced hash, and a filter eliminates tuples excluded in all subsamples:
\begin{equation}\label{eq:pac-select-rewrite}
\sigma_\phi(T_1 \bowtie_\theta T_2)
\;\longmapsto\;
\sigma_{h' \ne 0}\!\Bigl(
  \pi_{\ldots,\;\mathsf{pac\_select}(h,\,\mathbf{r})\;\mathrm{AS}\;h'}
  \bigl(T_1 \times T_2\bigr)
\Bigr).
\end{equation}
The outer aggregate then receives $h'$ in place of the original hash~$h$.

\vspace*{0mm}\noindent{\bf Correlated subqueries.}
When a correlated subquery contains a PAC aggregate, the inner and outer contexts each require an independently derived hash [todo- is this correct?].
The compiler inserts a separate FK join chain for the subquery branch, and each aggregate --- inner and outer --- receives its own hash expression.
The inner aggregate produces a counter vector
($\mathsf{pac\_agg\_ctr}$),
which is returned to the outer context at the correlation point.
The outer expression then applies a categorical rewrite as described above.

\vspace*{0mm}\noindent{\bf Mark joins (\textsc{in}/\textsc{exists}).}
\texttt{IN} and \texttt{EXISTS} subqueries are internally represented as
semi-joins ($\ltimes$) or mark joins.
When the semi-join condition references a PAC aggregate result, the
compiler converts the semi-join to a cross product with a PAC-aware
filter, following the pattern of Equation~\ref{eq:pac-select-rewrite}:
\begin{equation}\label{eq:mark-join}
T_1 \ltimes_\theta T_2
\;\longmapsto\;
\sigma_{h' \ne 0}\!\Bigl(
  \pi_{\ldots,\;\mathsf{pac\_select}(h,\,\mathbf{b})\;\mathrm{AS}\;h'}
  \bigl(T_1 \times T_2\bigr)
\Bigr),
\end{equation}
where $\mathbf{b}$ is the boolean counter vector from evaluating~$\theta$
across the $m$ subsamples.
When no outer aggregate exists, the construction simplifies to
$\sigma_{\mathsf{pac\_filter}(\mathbf{b})}(T_1 \times T_2)$.

\vspace*{0mm}\noindent{\bf TopK rewrite.}
\label{sec:topk-rule}
When $\mathsf{top}_k$ orders by a PAC aggregate result, ranking by noised
values would distort the ordering, since noise is calibrated for
output release rather than for internal decisions.
The compiler separates ranking from noising through a three-phase rewrite.
First, the aggregate produces the full counter vector~$\mathbf{c}$
via $\mathsf{pac\_agg\_ctr}$.
Second, $\mathsf{top}_k$ orders by the \emph{unnoised mean}
$\mathsf{pac\_mean}(\mathbf{c}) = \frac{1}{m}\sum_{j=1}^m c_j$,
which provides the best unbiased estimate of the true ranking without
consuming privacy budget.
Third, a final projection applies $\mathsf{pac\_noised}(\mathbf{c})$ to
produce the noised output exclusively for the selected rows:
\begin{equation}\label{eq:topk}
\begin{split}
\mathsf{top}_k^{\mathsf{pac\_agg}(\cdot)}
\;\longmapsto\;
&\pi_{\ldots,\;\mathsf{pac\_noised}(\mathbf{c})}\!\Bigl(
  \mathsf{top}_k^{\mathsf{pac\_mean}(\mathbf{c})}\!\bigl(\\
  &\quad\gamma_{G,\;\mathsf{pac\_agg\_ctr}(h,\,e)\;\mathrm{AS}\;\mathbf{c}}(T)
  \bigr)\Bigr).
\end{split}
\end{equation}

%% ----------------------------------------------------------------
\subsection{Equivalence}
\label{sec:equivalence}
We now establish that our single-query bitslice rewrite produces the same output distribution as PAC-DB's $m$-fold execution.

\begin{lemma}[Sampling Equivalence]\label{lem:sampling}
If $H$ is modeled as a uniformly random function, then for each PU
identifier~$u$ and bit position $j \in [1, m]$, the bit $H(u)[j]$ is an
independent $\mathrm{Bernoulli}(\frac{1}{2})$ random variable.
Consequently, the hash-based subsample
$S_j = \{t \in T : H(\mathsf{pu}(t))[j] = 1\}$
has the same distribution as the random 50\% PU sample used by PAC-DB.
\end{lemma}

\begin{proof}
Under the random oracle model, each output bit of $H$ is independent and
uniformly distributed over $\{0, 1\}$.
The indicator $\mathbb{1}[H(u)[j] = 1]$ therefore equals~1 with
probability exactly $\frac{1}{2}$ for every PU identifier~$u$ and every
bit position~$j$, independently across both dimensions.
This is precisely the sampling scheme used by PAC-DB, where each PU is
included in each subsample independently with probability~$\frac{1}{2}$.
\end{proof}

\begin{lemma}[Aggregation Equivalence]\label{lem:aggregation}
For any aggregation function~$\mathsf{agg}$ and expression~$e$, the
$j$-th counter of the bitslice aggregate equals the standard aggregate
evaluated on the $j$-th subsample:
\begin{equation}\label{eq:agg-equiv}
\mathsf{pac\_agg\_ctr}\!\bigl(H(\mathsf{pu}),\,e\bigr)[j]
\;=\;
\mathsf{agg}\!\bigl(\{e(t) : t \in S_j(T)\}\bigr).
\end{equation}
\end{lemma}

\begin{proof}
By definition (Equation~\ref{eq:counter}), counter~$j$ accumulates
contributions from exactly those tuples satisfying
$H(\mathsf{pu}(t))[j] = 1$, which is the set $S_j(T)$.
By Lemma~\ref{lem:sampling}, this set has the same distribution as
PAC-DB's $j$-th subsample.
For join elimination, referential integrity guarantees that
$T_k.fk_U = U.\mathsf{pk}$ for every matching tuple,
so $H(T_k.fk_U) = H(U.\mathsf{pk})$ and the subsample assignment is
identical whether computed from the foreign key or the primary key.
\end{proof}

\begin{lemma}[Categorical Equivalence]\label{lem:categorical}
Let $\phi$ be a boolean expression and
$b_j = \phi(c_j)$ for $j = 1, \ldots, m$,
where $c_j$ is the $j$-th subsample's aggregate result.
Then:
\emph{(i)}~$\mathsf{pac\_filter}(\mathbf{b})$ returns
$\mathsf{true}$ with probability $\frac{1}{m}\sum_j b_j$,
equal to the probability of the filter holding on a randomly chosen
PAC-DB subsample;
\emph{(ii)}~an outer aggregate using the reduced hash
$\mathsf{pac\_select}(h, \mathbf{b})$ computes, for each subsample~$j$,
the aggregate over exactly those rows in $S_j$ that satisfy $\phi$
within~$S_j$---identical to PAC-DB's per-subsample evaluation.
\end{lemma}

\begin{proof}
For part~\emph{(i)}: PAC-DB selects $k \xleftarrow{\$} [1,m]$ and returns
$b_k$; the probability $P(b_k{=}1) = \frac{1}{m}\sum_j b_j$ matches
$\mathrm{popcount}(\mathbf{b})/m$ by definition.
%
For part~\emph{(ii)}: the reduced hash
$h' = h \;\mathsf{AND}\; \mathbf{b}$ has
$h'[j] = H(\mathsf{pu})[j] \,\land\, b_j$.
The outer aggregate's counter~$j$ accumulates contributions from tuples
where both $H(\mathsf{pu})[j] = 1$ (membership in~$S_j$) and
$b_j = 1$ (filter holds in~$S_j$).
In PAC-DB, subsample~$j$ evaluates the filter on $S_j$'s own data,
producing the same partition of contributing tuples.
\end{proof}

\begin{theorem}[End-to-End Equivalence]\label{thm:equivalence}
For any supported query~$Q$,
$\mathsf{PacRewrite}(Q)$ produces the same output distribution as
$\mathcal{N}^{\mathsf{pac}(\beta)}\!\bigl(Q(S_1), \ldots, Q(S_m)\bigr)$.
\end{theorem}

\begin{proof}
We proceed by structural induction on the query plan.

\emph{Base case.}
Consider a simple aggregation $Q = \gamma_{G,\,\mathsf{agg}(e)}\!(\sigma_p(T))$.
By Lemma~\ref{lem:sampling}, the hash-based subsamples have the same
distribution as PAC-DB's random subsamples.
By Lemma~\ref{lem:aggregation}, the bitslice counter values match the
per-subsample aggregate results.
Since $\mathsf{pac\_noised}$ applies the identical noise mechanism
$\mathcal{N}^{\mathsf{pac}(\beta)}$ to these counter values, the output
distributions are equal.

\emph{Inductive step.}
Each translation rule preserves the invariant that the $m$ counter values
correspond to the $m$ PAC-DB subsample results.
Standard selections and projections on non-aggregate attributes commute
with subsampling: $\sigma_p(S_j(T)) = S_j(\sigma_p(T))$ when $p$ does
not reference~$\mathsf{pu}$, and analogously for projections.
Categorical rewrites evaluate expressions elementwise over counters,
which by Lemma~\ref{lem:categorical} is equivalent to evaluating the
expression on each subsample independently.
Correlated subqueries maintain independent hash derivations for inner
and outer contexts, but both use the same hash function~$H$, so
subsample~$j$ in the inner query corresponds to subsample~$j$ in the
outer query.
Mark join rewrites restructure the semi-join while preserving
per-subsample filter semantics through $\mathsf{pac\_select}$
(Lemma~\ref{lem:categorical}\emph{(ii)}).
The TopK rewrite selects rows by unnoised means and applies noise as a
post-processing step to the same counter values;
since noise application is applied after a deterministic selection,
the output has the same distribution as noising the PAC-DB result.
CTEs share the same hash across all references, ensuring consistent
subsample assignment.
\end{proof}


%% ----------------------------------------------------------------
\subsection{\textsf{PacRewrite} Algorithm}
\label{sec:algorithm-examples}

Algorithm~\ref{alg:pac-rewrite} formalizes the compilation procedure as
a single recursive function over the relational algebra tree.
The function performs a top-down pass to insert PU joins and derive hash expressions, recurses into the children, and then applies a bottom-up pass to replace aggregates and rewrite categorical expressions.
                      
\begin{algorithm}[t]                                                                     
  \small
  \caption{The \textsf{PacRewrite} algorithm. Top-down: insert PU joins and derive hash expressions.  
    Bottom-up: replace aggregates and rewrite categorical expressions.}                                                    
  \label{alg:pac-rewrite}                                   
  \begin{algorithmic}[1]
  \Function{PacRewrite}{node $n$, PU metadata $\mathcal{M}$}
    \Comment{\textit{--- Top-down phase}}
    \If{$n = \mathrm{Scan}(T)$ \textbf{and} $\mathrm{FKPath}(T,U)\in\mathcal{M}$
        \textbf{and} no join to $U$ in plan}
      \State $T \xrightarrow{fk_1} T_1 \xrightarrow{fk_2} \cdots
             \xrightarrow{fk_k} U \gets \mathrm{FKPath}(T,U)$
      \State $n \gets n \bowtie_{fk_1}
             \pi_{\mathsf{pk}_1,fk_2}(\mathrm{Scan}(T_1))
             \bowtie_{fk_2} \cdots$
             \Comment{PU join addition}
      \State $n \gets \pi_{\mathrm{cols}(n),\;H(T_k.fk_U)\;\mathrm{AS}\;h}(n)$
             \Comment{hash from last FK}
    \EndIf
    \If{$n = \mathrm{CTE}[\mathrm{body}]$ \textbf{and} body refs.\ PU tables}
      \State $\mathrm{body} \gets
             \Call{PacRewrite}{\mathrm{body},\mathcal{M}}$
      \State $n \gets \mathrm{CTE}[
             \pi_{\mathrm{cols}(\mathrm{body}),h}(\mathrm{body})]$
             \Comment{CTE hash propagation}
    \EndIf
    \Comment{\textit{--- Recurse on children}}
    \For{each child $n_i$ of $n$}
      \State $n_i \gets \Call{PacRewrite}{n_i,\mathcal{M}}$
    \EndFor
    \Comment{\textit{--- Bottom-up phase}}
    \If{$n = \gamma_{G,\mathsf{agg}(e)}(T)$ \textbf{and} $T$ is PU-linked}
      \State $h \gets$ hash column propagated from $T$
      \State $n \gets \textbf{if}\ \text{categorical ctx.}\
             \textbf{then}\ \gamma_{G,\,\mathsf{pac\_agg\_ctr}(h,e)}(T)$
      \Statex \hspace{3.1em}$\textbf{else}\
             \gamma_{G,\,\mathsf{pac\_agg}(h,e)}(T)$
    \EndIf
    \If{$n \in \{\sigma_\phi, \pi_\phi\}$ \textbf{and}
        $\phi$ refs.\ $\mathsf{pac\_agg\_ctr}$}
      \State $\mathbf{r} \gets
             \langle\phi(c_1),\ldots,\phi(c_m)\rangle$
             \Comment{elementwise}
      \If{$n = \sigma$ \textbf{and} outer agg.\ exists}
        \State $h' \gets \mathsf{pac\_select}(h,\mathbf{r})$
        \State $n \gets \sigma_{h'\ne 0}(
               \pi_{\ldots,h'}(T_1\times T_2))$
      \ElsIf{$n = \sigma$}
        \State $n \gets \sigma_{\mathsf{pac\_filter}(\mathbf{r})}(
               n.\mathrm{child})$
      \ElsIf{$n = \pi$}
        \State $n \gets \pi_{\ldots,\mathsf{pac\_noised}(\mathbf{r})}(
               n.\mathrm{child})$
      \EndIf
    \EndIf
    \If{$n \in \{\bowtie_\theta, \ltimes_\theta\}$ \textbf{and}
        $\theta$ involves $\mathsf{pac\_agg\_ctr}$}
      \State eval $\theta$ elementwise $\to\mathbf{b}$
      \State $n \gets \sigma_{h'\ne 0}(\pi_{\ldots,
             \mathsf{pac\_select}(h,\mathbf{b})\,\mathrm{AS}\,h'}
             (T_1\times T_2))$
    \EndIf
    \If{$n = \mathsf{top}_k$ ordered by $\mathsf{pac\_agg}$}
      \State convert to $\mathsf{pac\_agg\_ctr}\to\mathbf{c}$;
             apply Eq.~\ref{eq:topk}
    \EndIf
    \State \Return $n$
  \EndFunction
  \end{algorithmic}
  \end{algorithm}


\vspace*{0mm}\noindent{\bf Example 1: TPC-H Q15 (CTE, fused aggregation).}
Q15 identifies the supplier with the highest revenue from shipped lineitems
in a given quarter.
Let $L = \mathsf{lineitem}$, $O = \mathsf{orders}$,
$C = \mathsf{customer}$, $S = \mathsf{supplier}$, and
$p_{\mathit{ship}}$ denote the shipdate predicate.
We abbreviate column names for space
($l\_ep = \mathsf{l\_extendedprice}$, $l\_disc = \mathsf{l\_discount}$,
etc.).
The original (non-private) query defines a revenue CTE and selects the top supplier:
\begin{align}
R &= \gamma_{\mathsf{l\_suppkey},\;\mathsf{SUM}(l\_ep \cdot (1 - l\_disc))\;\mathrm{AS}\;r}
    \!\bigl(\sigma_{p_{\mathit{ship}}}(L)\bigr), \label{eq:q15-orig-cte}\\
Q_{15} &=
  \pi_{\mathsf{s\_suppkey},\,\mathsf{s\_name},\,\mathsf{s\_addr},\,\mathsf{s\_phone},\,r}\!\bigl(
  \sigma_{r = \gamma_{\mathsf{MAX}(r)}(R)}(S \bowtie R)\bigr). \label{eq:q15-orig}
\end{align}
Note that the original scans only $L$ --- no join to $O$ or $C$ is needed.

Under PAC-DB, the customer PU must be tracked, so lineitem is joined with orders and customer before subsampling.
For each $j \in [1,m]$, the subsample operator $\mathcal{S}_j$ is
applied and the CTE is materialized per subsample:
\begin{equation}\label{eq:q15-pacdb}
R_j = \gamma_{\mathsf{l\_suppkey},\;\mathsf{SUM}(l\_ep \cdot (1 - l\_disc))\;\mathrm{AS}\;r}
      \!\bigl(\sigma_{p_{\mathit{ship}}}
      (\mathcal{S}_j(L \bowtie O \bowtie C))\bigr).
\end{equation}
The outer query
$\pi_{\ldots}\!\bigl(
  \sigma_{r = \gamma_{\mathsf{MAX}(r)}(R_j)}(S \bowtie R_j)
\bigr)$
is evaluated per subsample, and the noise mechanism
$\mathcal{N}^{\mathsf{pac}(\beta)}$ is applied
across the $m$ results.
This requires joining lineitem, orders, \emph{and} customer in every
execution to enable subsample filtering on the PU.

Our rewrite eliminates both the $m$-fold execution and the join to
customer.
The compiler applies three rules:
\emph{(i)}~join addition inserts the join
$L \bowtie_{l\_ok = o\_ok} O$ to reach the FK column
$\mathsf{o\_custkey}$;
\emph{(ii)}~join elimination observes that
$H(\mathsf{o\_custkey}) = H(\mathsf{c\_custkey})$ by referential
integrity (Equation~\ref{eq:join-elim}), so the join to $C$ is skipped;
\emph{(iii)}~aggregate replacement transforms $\mathsf{SUM}$ into the
fused $\mathsf{pac\_sum}$.
The CTE rule ensures the hash is exposed to all consumers.
The rewritten revenue CTE becomes:
\begin{equation}\label{eq:q15-ours}
\widehat{R} = \gamma_{\mathsf{l\_suppkey},\;
  \mathsf{pac\_sum}(H(\mathsf{o\_ck}),\;l\_ep \cdot (1 - l\_disc))
  \;\mathrm{AS}\;r}
  \!\bigl(\sigma_{p_{\mathit{ship}}}(L \bowtie_{l\_ok = o\_ok} O)\bigr),
\end{equation}
and the outer query is
$\pi_{\ldots}\!\bigl(
  \sigma_{r = \gamma_{\mathsf{MAX}(r)}(\widehat{R})}
  (S \bowtie \widehat{R})\bigr)$.
The comparison $r = \mathsf{MAX}(r)$ operates on already-noised scalars
materialized by the CTE; this is deterministic post-processing and
consumes no additional privacy budget.

\vspace*{0mm}\noindent{\bf Example 2: TPC-H Q17
(categorical filter, correlated subquery).}
Q17 computes the average yearly revenue lost due to small-quantity orders,
where ``small'' is defined relative to the per-part average.
Let $P = \mathsf{part}$ and let $p_{\mathit{brand}}$ denote the brand/container
predicate.
The original query applies a correlated subquery to filter lineitems whose
quantity falls below $20\%$ of the per-part average:
\begin{equation}\label{eq:q17-orig}
Q_{17} = \gamma_{\mathsf{SUM}(l\_ep)/7}\!\Bigl(
  \sigma_{p_{\mathit{brand}} \,\land\,
    l\_qty < 0.2 \cdot
    \gamma_{\mathsf{AVG}(l\_qty)}
    (\sigma_{l\_pk = p\_pk}(L))}
  \!\bigl(L \bowtie P\bigr)
\Bigr).
\end{equation}

Under PAC-DB, the subsampled lineitem is pre-joined with the PU:
$T_j = \mathcal{S}_j(L \bowtie O \bowtie C)$.
Both the outer $\mathsf{SUM}$ and the correlated $\mathsf{AVG}$ operate
on the \emph{same} subsample~$T_j$, ensuring consistent filter evaluation
within each subsample:
\begin{equation}\label{eq:q17-pacdb}
\gamma_{\mathsf{SUM}(l\_ep)/7}\!\Bigl(
  \sigma_{p_{\mathit{brand}} \,\land\,
    l\_qty < 0.2 \cdot
    \gamma_{\mathsf{AVG}(l\_qty)}
    (\sigma_{l\_pk = p\_pk}(T_j))}
  \!\bigl(T_j \bowtie P\bigr)
\Bigr).
\end{equation}
After $m$ executions, the noise mechanism is applied.

Our rewrite replaces the $m$-fold execution with categorical functions.
Five rules apply:
\emph{(i)}~join addition and elimination insert joins to orders in both
the outer and inner (correlated) contexts, skipping customer;
\emph{(ii)}~the correlated subquery rule inserts a separate FK join
chain for the subquery, with alias $O_{\mathit{sub}}$;
\emph{(iii)}~the inner $\mathsf{AVG}$ is replaced by the counter variant
$\mathsf{pac\_avg\_ctr}$, since its result participates in a comparison;
\emph{(iv)}~the categorical rewrite transforms the predicate
$l\_qty < 0.2 \cdot \mathsf{AVG}(\ldots)$
into the algebraically equivalent
$\mathsf{pac\_filter\_lt}(5 \cdot l\_qty,\;\mathbf{c})$,
which evaluates the comparison against each counter value and returns
true with probability $\mathrm{popcount}(\mathbf{b})/m$;
\emph{(v)}~the outer $\mathsf{SUM}$ is replaced by the fused
$\mathsf{pac\_sum}$.
The rewritten query reads:
\begin{equation}\label{eq:q17-ours}
\begin{split}
A &= \gamma_{\mathsf{pac\_avg\_ctr}(H(\mathsf{o\_ck}^{\mathit{sub}}),\,l\_qty)}
     (\sigma_{l\_pk = p\_pk}(L_{\mathit{sub}} \bowtie O_{\mathit{sub}})) \\
&\gamma_{\mathsf{pac\_sum}(H(\mathsf{o\_ck}),\,l\_ep)/7}\!\Bigl(
  \sigma_{p_{\mathit{brand}} \,\land\,
    \mathsf{pac\_filter\_lt}(5 \cdot l\_qty,\; A)}
  (L \bowtie P \bowtie O)
\Bigr).
\end{split}
\end{equation}


